Learning Multimodal Latent Generative Models with Energy-Based Prior

Multimodal generative models have recently gained significant attention for their ability to learn representations across various modalities, enhancing joint and cross-generation coherence. However, most existing works use standard Gaussian or Laplacian distributions as priors, which may struggle to capture the diverse information inherent in multiple data types due to their unimodal and less informative nature. Energy-based models (EBMs), known for their expressiveness and flexibility across various tasks, have yet to be thoroughly explored in the context of multimodal generative models. In this paper, we propose a novel framework that integrates the multimodal latent generative model with the EBM. Both models can be trained jointly through a variational scheme. This approach results in a more expressive and informative prior, better-capturing of information across multiple modalities. Our experiments validate the proposed model, demonstrating its superior generation coherence.

==> sec/4_exp_sy_nomst.tex <==
\section{Experiments}
\label{sec:exp}
In this section, we conduct various experiments to demonstrate the expressiveness of the EBM prior in capturing shared latent information across multimodalities more effectively than less-informative unimodal priors (e.g., Gaussian or Laplacian priors). In our experiments, we follow the prior arts \cite{pang2020learning} and train our model on standard multimodal datasets, such as the PolyMNIST \cite{sutter2021generalized} and MNIST-SVHN \cite{shi2019variational}. We evaluate the performance of our model in terms of joint coherence (\cref{sec:joint-coherence}) and cross coherence (\cref{sec:cross-coherence}). Additionally, we demonstrate the applicability and flexibility of the proposed method, showing its capacity for generalization to various factorizations (\cref{sec:model-generation}), including the incorporation of model-specific factors \cite{palumbo2023mmvae+}. And we visualize the Markov transition on image synthesis and corresponding
generated text applied to Caltech UCSD Birds (CUB) dataset \cite{wah2011caltech}. Furthermore, we conduct ablation studies (\cref{sec:ablation-studies}) to gain a deeper understanding of our approach. We provided our code in  
\url{https://github.com/syyuan2021/Learning-Multimodal-Latent-Generative-Models-with-EBM}\\

\noindent\textbf{Baseline Method.} For comparisons, our direct baselines include MVAE\cite{wu2018multimodal} and MMVAE \cite{shi2019variational}, and we also compare with recent mmJSD \cite{sutter2020multimodal}, MoPoE \cite{sutter2021generalized}, MVTACE\cite{hwang2021multi} and MMVAE$+$ \cite{palumbo2023mmvae+} that are developed based on the foundation methods of \textit{product-of-expert} \cite{wu2018multimodal} and \textit{mixture-of-expert} \cite{shi2019variational}. For a fair comparison, we adopt the same generation and inference network structures, as well as the pre-trained classifiers from \cite{sutter2021generalized} for PolyMNIST, and follow \cite{shi2019variational}'s implementation to train the classifier for MNIST-SVHN.\\

\subsection{Joint Coherence}\label{sec:joint-coherence}
With a set of $m$ modalities, we asses our model in generating \textit{unconditional} image synthesis that maintains strong coherence across different modalities. If the EBM prior is well-learned, it should be capable of sampling the latent variables that capture semantic representations and thus generating the image synthesis semantically consistent between multimodalities. We measure such coherence by computing the classification accuracy of generated images of each modality with corresponding classifiers. Higher accuracy indicates better consistency between predicted categories of multimodal synthesis.\\

We report the quantitative results in Tab. \ref{tab:gen-base}, where our EBM prior shows superior performance compared to baseline models. Both numerically and visually, the EBM prior successfully captures complex latent representations, whereas the unimodal prior (Laplacian) is less expressive and limited in modeling meaningful semantic representations. Synthesis of joint generation can be found in Fig. \ref{fig:joint-results-base}. \\

\begin{table}[h]
    \centering
    \caption{Accuracy of Joint Coherence and Cross Coherence for PolyMNIST and MNIST-SVHN datasets. The PolyMNIST results for MVAE are referenced from \cite{palumbo2023mmvae+}, and MNIST-SVHN results for MVAE are referenced from \cite{shi2019variational}. MMVAE$^{*}$ refers to \textit{mixture of expert} without important sampling. }
    \label{tab:gen-base}
    \resizebox{0.8\columnwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c}
        \toprule
        \multicolumn{3}{c|}{Joint Coherence} & \multicolumn{3}{c}{Cross Coherence} \\
        \midrule
        \multirow{2}{*}{Model} & \multirow{2}{*}{PolyMNIST}  & \multirow{2}{*}{MNIST-SVHN} & \multirow{2}{*}{PolyMNIST} & \multicolumn{2}{c}{MNIST-SVHN} \\
        \cmidrule(lr){5-6}
        & & & & M->S & S->M \\
        \midrule
        Ours &\textbf{\textcolor{blue}{0.746} (0.735)} $\uparrow$ &\textbf{\textcolor{blue}{0.419} (0.412)} $\uparrow$ &\textbf{\textcolor{blue}{0.853} (0.857)} $\uparrow$ &\textbf{\textcolor{blue}{0.237} (0.195)} $\uparrow$ &\textbf{\textcolor{blue}{0.657} (0.657)} $\uparrow$\\
        \midrule
        MVAE &0.080 &0.127 &0.298 &0.095 &0.093 \\
        \midrule
        MMVAE$^{*}$ &0.232 &0.215 &0.844 &0.169 &0.523 \\
        \bottomrule
    \end{tabular}
    }
\end{table}

\begin{figure}[h]
\captionsetup{singlelinecheck=off}
\captionsetup[subfigure]{singlelinecheck=on}
    \centering   
    \captionbox{Qualitative Results of Joint Generation on  MNIST-SVHN (top) and PolyMNIST (bottom)) \label{fig:joint-results-base}}[0.9\textwidth]{
            \subcaptionbox{\textcolor{blue}{Updated EBM Prior}}[0.42\textwidth][l]{%
                   \includegraphics[width=0.197\textwidth]{images/gen_samples_ebm_1_003.png}%
                  \includegraphics[width=0.197\textwidth]{images/gen_samples_ebm_0_003.png}%
               \\    \includegraphics[width=0.394\textwidth]{images/update_poly_base_joint.png}%
            }
            \subcaptionbox{Unimodal Prior: MMVAE$^{*}$}[0.42\textwidth][l]{%
               \includegraphics[width=0.199\textwidth]{images/mmvae_gen_samples_1.png}%
              \includegraphics[width=0.199\textwidth]{images/mmvae_gen_samples_0.png}%
               \\    \includegraphics[width=0.398\textwidth]{images/poly_joint_base_uni.png}%
            }
        }
        {
            \subcaptionbox{Previour EBM Prior}[0.42\textwidth][l]{%
                   \includegraphics[width=0.197\textwidth]{images/ebm_gen_samples_1.png}%
                  \includegraphics[width=0.197\textwidth]{images/ebm_gen_samples_0.png}%
               \\    \includegraphics[width=0.394\textwidth]{images/poly_joint_base_ours.png}%
            }
            \subcaptionbox{Unimodal Prior: MMVAE$^{*}$}[0.42\textwidth][l]{%
               \includegraphics[width=0.199\textwidth]{images/mmvae_gen_samples_1.png}%
              \includegraphics[width=0.199\textwidth]{images/mmvae_gen_samples_0.png}%
               \\    \includegraphics[width=0.398\textwidth]{images/poly_joint_base_uni.png}%
            }
        }
\end{figure}

% \begin{figure}[h]
% \captionsetup{singlelinecheck=off}
% \captionsetup[subfigure]{singlelinecheck=on}
%     \centering   
%     \captionbox{Qualitative Results of Joint Generation on  MNIST-SVHN (top) and PolyMNIST (bottom)) \label{fig:joint-results-base}}[0.9\textwidth]{
%             \subcaptionbox{EBM Prior}[0.42\textwidth][l]{%
%                    \includegraphics[width=0.197\textwidth]{images/ebm_gen_samples_1.png}%
%                   \includegraphics[width=0.197\textwidth]{images/ebm_gen_samples_0.png}%
%                \\    \includegraphics[width=0.394\textwidth]{images/poly_joint_base_ours.png}%
%             }
%             \subcaptionbox{Unimodal Prior: MMVAE$^{*}$}[0.42\textwidth][l]{%
%                \includegraphics[width=0.199\textwidth]{images/mmvae_gen_samples_1.png}%
%               \includegraphics[width=0.199\textwidth]{images/mmvae_gen_samples_0.png}%
%                \\    \includegraphics[width=0.398\textwidth]{images/poly_joint_base_uni.png}%
%             }
%         }
% \end{figure}

\subsection{Cross Coherence}\label{sec:cross-coherence}
Next, we evaluate our model in cross-modal generation. Cross-modal generation is to generate image synthesis from input modality $\rvx^{(i)}$ to target modality $\rvx^{(j)}$ ($i \ne j$). Specifically, given input $\rvx^{(i)}$, we first obtain inferred latent vector $\rvz \sim q_\phi(\rvz|\rvx^{(i)})$ and then generate synthesis via generation model $\rvx^{(j)} \sim p_{\beta_{j}}(\rvx^{(j)}|\rvz)$. With our EBM prior, the inference and generation model can be learned to integrate both the modality bias and the energy-based refinement and thus the latent vectors inferred from $\rvx^{(i)}$ carry the semantic representation shared with $\rvx^{(j)}$, leading to coherent input $\rvx^{(i)}$ and output $\rvx^{(j)}$. To measure the coherence, we compute the classification accuracy (same classifiers used in Sec. \ref{sec:joint-coherence}) of the predicted category of $\rvx^{(j)}$ and true category of $\rvx^{(i)}$. Higher accuracy means both the $\rvx^{(i)}$ and $\rvx^{(j)}$ share higher similarity in semantic features (e.g., digit classes in PolyMNIST). The results can be found in Tab. \ref{tab:gen-base}, in which the proposed method can render competitive performance compared to the baseline methods, suggesting the effectiveness of our EBM prior in multimodalities learning.

\subsection{Model Generalization}\label{sec:model-generation}
This paper studies learning a novel framework for foundation multimodal latent generative models, such as MVAE and MMVAE, which serve as the building blocks of various recent works. In this section, we highlight the applicable capability of the proposed method toward other prior advances \cite{palumbo2023mmvae+}. These advances usually factorize additional \textit{modal-specific prior} or \textit{modal-subset} to benefit the model complexity in learning the complex multimodalities. In particular, MMVAE$+$ develop their latent generative model as
\begin{equation}
\label{mmvae+}
\begin{aligned} 
    p_{\beta}(\rvX, \rvz,\rvW) = p_{\beta}(\rvX|\rvz,\rvW)p_0(\rvz)p_0(\rvW)
\end{aligned}
\end{equation}
where the prior model $p_0(\rvW)$ is modal-specific (i.e., $\rvW=\{\rvw^{(1)},\dots,\rvw^{(m)}\}$) and is introduced to improve the expressivity of the whole prior model (compared to Eqn. \ref{joint}. However, the shared latent representation is still modelled by $p_0(\rvz)$, which is assumed to be Laplacian and can be less informative.\\

\vspace{-5mm}
\begin{table}[h]
\centering
\setlength{\belowcaptionskip}{-0.5pt}%
% \setlength{\abovecaptionskip}{-20pt}%
\caption{Accuracy of Joint Coherence and Cross Coherence for PolyMNIST. Results of MMVAE$+$, MoPoE, MVTCAE, and mmJSD are reported in \cite{palumbo2023mmvae+}. Ours$+$ refers to generalizing our model with modality-specific priors.}
\label{tab:gen-advance}
\resizebox{0.6\columnwidth}{!}{
\begin{tabular}{c|c|c}
    \toprule
    Model 	& Joint Coherence & Cross Coherence \\
    \midrule
    Ours$+$ &\textbf{\textcolor{blue}{0.878} (0.848) $\uparrow$}  &\textbf{\textcolor{blue}{0.897} (0.889) $\uparrow$} \\
    \midrule
    MMVAE$+$ &0.344 &0.869  \\
    MoPoE &0.141 &0.720  \\
    MVTCAE  &0.003 &0.591 \\
    mmJSD   &0.060 &0.778  \\
    \bottomrule
\end{tabular}
}
\end{table}
\vspace{-5mm}

\begin{figure}[ht]
    \centering
    \begin{subfigure}[]{0.49\textwidth}
    \includegraphics[height=0.15\textheight]{images/updated_ebm_joint_adv0.png}
    \caption{\textcolor{blue}{Updated EBM Prior}}
    % \label{fig:joint_mmvae_ours}
    \end{subfigure}
    \begin{subfigure}[]{0.49\textwidth}
    % \centering
    \includegraphics[height=0.15\textheight]{images/poly_joint_ours.png}
    \caption{Previous EBM Prior}
    % \label{fig:joint_mmvae_plus}
    \end{subfigure}   
    \begin{subfigure}[]{0.49\textwidth}
    \includegraphics[height=0.15\textheight]{images/updated_ebm_joint_adv0.png}
    \caption{\textcolor{blue}{Updated EBM Prior}}
    % \label{fig:joint_mmvae_ours}
    \end{subfigure}
    \begin{subfigure}[]{0.49\textwidth}
    % \centering
    \includegraphics[height=0.15\textheight]{images/poly_joint_iclr23.png}
    \caption{Unimodal Prior}
    % \label{fig:joint_mmvae_plus}
    \end{subfigure}   
    \caption{Qualitative results of Joint Generation on PolyMNIST}
    \label{fig:joint-results-advance}  
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}{1\textwidth}
            \centering 
            \includegraphics[width=0.15\textwidth,height=0.335\textheight]{images/update_ebm_adv.png}
            \includegraphics[width=0.15\textwidth,height=0.335\textheight]{images/cross_gen_ours_advance.png}
            \includegraphics[width=0.15\textwidth,height=0.335\textheight]{images/cross_gen_mmvae+.png}
            \includegraphics[width=0.15\textwidth,height=0.335\textheight]{images/cross_gen_mopoe.png}
            \includegraphics[width=0.15\textwidth,height=0.335\textheight]{images/cross_gen_mmjsd.png}
            \includegraphics[width=0.15\textwidth,height=0.335\textheight]{images/cross_gen_mvtcae.png}
    \end{subfigure}
    \caption{Qualitative results of Cross Generation on PolyMNIST. From left to right, cross generation results are from (a) \textcolor{blue}{Updataed EBM prior} (b) Previous EBM prior, (c) MMVAE$+$, (d) MoPoE, (e) mmJSD, and (f) MVTCAE. }
    \label{fig:cross-results-advance}
\end{figure}

% \begin{figure}[h]
%     \centering
%     \begin{subfigure}{1\textwidth}
%             \centering 
%             \includegraphics[width=0.19\textwidth,height=0.4\textheight]{images/cross_gen_ours_advance.png}
%             \includegraphics[width=0.19\textwidth,height=0.4\textheight]{images/update_ebm_adv.png}
%             \includegraphics[width=0.19\textwidth,height=0.4\textheight]{images/cross_gen_mmvae+.png}
%             \includegraphics[width=0.19\textwidth,height=0.4\textheight]{images/cross_gen_mopoe.png}
%             \includegraphics[width=0.19\textwidth,height=0.4\textheight]{images/cross_gen_mmjsd.png}
%             \includegraphics[width=0.19\textwidth,height=0.4\textheight]{images/cross_gen_mvtcae.png}
%     \end{subfigure}
%     \caption{Qualitative results of Cross Generation on PolyMNIST. From left to right, cross generation results are from (a) EBM prior, (b) MMVAE$+$, (c) MoPoE, (d) mmJSD, and (e) MVTCAE. }
%     \label{fig:cross-results-advance}
% \end{figure}


\noindent\textbf{Generalization.} Our model is flexible and can be adapted to incorporate such a modal-specific factor, i.e., $p_{\beta,\alpha}(\rvX, \rvz, \rvW) = p_{\beta}(\rvX|\rvz, \rvW)p_{\alpha}(\rvz)p_{0}(\rvW)$, such that the shared latent representation is modelled by the proposed EBM prior $p_{\alpha}(\rvz)$, which can be multi-modal and more expressive than the unimodal prior model $p_0(\rvz)$. To examine the effectiveness, we follow MMVAE$+$ and train our model on PolyMNIST with the same network structures. We report the results of joint coherence and cross coherence in Tab. \ref{tab:gen-advance} and the qualitative results in Fig. \ref{fig:joint-results-advance} and Fig. \ref{fig:cross-results-advance}. \\

\noindent \textbf{Caltech UCSD Birds Dataset (CUB)}. To examine the scalability, we further train our model on the challenging multimodal dataset Caltech UCSD Birds (CUB)\cite{wah2011caltech}. The proposed EBM can be viewed as an exponential tilting of the reference distribution and thus can correct the less informative prior model toward being more expressive. In this section, we intend to demonstrate the expressivity of our EBM prior in correcting the unimodal prior model. In practice, we utilize the same network structure and train MMVAE$+$ on CUB, and then we learn our EBM prior with the pre-trained generation and inference model. If our EBM prior can be learned well, the quality of synthesis generated by our EBM prior samples should be better than samples of the unimodal prior.

For illustration, we visualize the Markov chain transition during Langevin dynamics on generated images and text in Fig. \ref{fig:cub_mcmc}. Specifically, the Markov chain transition starts from the latent drawn from the unimodal prior $p_0(\rvz)$ and then progresses as an iterative sampler for our EBM prior $p_\alpha(\rvz)$. It can be seen that the quality of image and text synthesis becomes better as the Langevin dynamics progresses and, more importantly, at the final step, the generated images and text render better semantic coherence, which further indicates the effectiveness of the proposed EBM prior.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.99\textwidth]{images/mcmc_v2.png}
    \caption{Visualization of Markov chain transition on image synthesis and corresponding generated text. \textbf{Left}: visualization of Markov chain transition where left column images are generated by \textit{unimodal} prior sample, and right column images are generated by \textit{EBM} prior sample. \textbf{Right}: jointly generated text corresponding to each row in left figure. The sentence at the top is generated by  \textit{unimodal} prior sample, and the sentence at the bottom is generated by \textit{EBM} prior sample.}
    \label{fig:cub_mcmc}
\end{figure}

\subsection{Ablation Studies}\label{sec:ablation-studies}
In the previous sections, we demonstrated the effectiveness of using an EBM prior in multimodal contexts, illustrating that our model can better capture complex data representations across different modalities. To further investigate our model's capabilities, we examine the impact of our EBM prior settings on performance through a series of experiments conducted on the PolyMNIST dataset.\\

\noindent \textbf{Energy-Based Model MCMC Steps:} We first examine the influence of the number of MCMC steps, denoted as $S$, when sampling the latent variables from EBM prior. We fixed the network architecture to consist of 4 layers with 400 hidden units each. As observed in the middle two rows of Tab. \ref{tab:abalation_poly}, a smaller number of MCMC steps results in poorer performance. However, increasing the number of MCMC steps is computationally expensive, leading to a trade-off between computation time and model performance. \\

\noindent \textbf{Energy-Based Model Layers:} Then we examine whether more information transformation and interaction will increase coherence scores. So we fixed hidden dimension and Langevin steps while increase EBM layer $L$ from 4 to 6. As shown in the first two rows of Tab. \ref{tab:abalation_poly}, increasing the number of layers $L$ leads to better coherence results. \\

\noindent \textbf{Energy-Based Model Complexity:} 
Increasing the model dimension allows the model to learn more complex and representative features. To examine scalability, we increase the dimension of hidden units $D$ to investigate the performance impact of capacity in capturing and processing information. We maintain the number of layers at 4 and use 50 Langevin steps. As observed in the bottom two rows of Tab. \ref{tab:abalation_poly}, increasing the number of units results in better coherence performance. \\

\begin{table}[h]
\centering
\setlength{\belowcaptionskip}{-0.5pt}%
% \setlength{\abovecaptionskip}{-20pt}%
\caption{Ablation studies for energy-based models with different numbers of hidden units $D$, MCMC steps $S$, and network layers $L$.}
\label{tab:abalation_poly}
\resizebox{0.8\columnwidth}{!}{
\begin{tabular}{c|c|c}
    \toprule
    Model 	& Joint Coherence & Cross Coherence \\
    \midrule
    Ours (D=200, L=4, S=50) &0.580 &0.854 \\
    Ours (D=200, L=6, S=50) &0.682 &0.840 \\
    \midrule
    Ours (D=400, L=4, S=30) &\textcolor{blue}{0.683} (0.641) & \textcolor{blue}{0.845} (0.825) \\
    Ours (D=400, L=4, S=50) &\textbf{\textcolor{blue}{0.746} (0.735)} &\textbf{\textcolor{blue}{0.853} (0.857)} \\
    \midrule
    Ours (D=200, L=4, S=50) &0.580 &0.854 \\
    Ours (D=400, L=4, S=50) &\textbf{\textcolor{blue}{0.746} (0.735)} &\textbf{\textcolor{blue}{0.853} (0.857)} \\
    \bottomrule
\end{tabular}
}
\end{table}

